The Debt-Inflation Channel of the German (Hyper-)Inflation

This paper studies how a large increase in the price level is transmitted to the real economy through firm balance sheets. Using newly digitized macro- and micro-level data from the German inflation of 1919-1923, we show that inflation led to a large reduction in real debt burdens and bankruptcies. Firms with higher nominal liabilities at the onset of inflation experienced a larger decline in interest expenses, a relative increase in their equity values, and higher employment during the inflation. The results are consistent with real effects of a debt-inflation channel that operates even when prices and wages are flexible.

==> output/tex/Tab_board_network_controls.tex <==
\begin{tabular}{l*{5}{c}}   \toprule  Dependent Variable & \multicolumn{5}{c}{ln(Employment)} \\    \cmidrule(lr){2-6}       
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         \\
\midrule
Liabl./Assets$_{i,1917}$ $\times$$\mathbf{1}_{t\geq1920}$&     42.8\sym{**} &     37.9\sym{**} &     39.5\sym{**} &     39.4\sym{**} &     42.5\sym{**} \\
                &   (18.0)         &   (18.5)         &   (18.1)         &   (18.6)         &   (18.2)         \\
Government $ $\times$$\mathbf{1}_{t\geq1920}&     3.57         &                  &                  &                  &     5.84         \\
                &   (4.63)         &                  &                  &                  &   (4.64)         \\
Reichsbank $\times$$\mathbf{1}_{t\geq1920}$&                  &    -7.76\sym{*}  &                  &                  &    -9.51\sym{*}  \\
                &                  &   (4.49)         &                  &                  &   (5.41)         \\
Hugo Stinnes $\times$$\mathbf{1}_{t\geq1920}$&                  &                  &    -0.21         &                  &     6.14         \\
                &                  &                  &   (3.54)         &                  &   (4.76)         \\
Bank  $\times$$\mathbf{1}_{t\geq1920} &                  &                  &                  &    -8.72\sym{*}  &    -9.65         \\
                &                  &                  &                  &   (4.91)         &   (6.44)         \\
\midrule
Observations    &     2148         &     2138         &     2138         &     2138         &     2138         \\
Number of Firms &      317         &      316         &      316         &      316         &      316         \\
\(R^2_{overall}\)&     0.97         &     0.97         &     0.97         &     0.97         &     0.97         \\
\(R^2_{within}\)&    0.054         &    0.058         &    0.051         &    0.056         &    0.067         \\
Year FE         &\checkmark         &\checkmark         &\checkmark         &\checkmark         &\checkmark         \\
Firm FE         &\checkmark         &\checkmark         &\checkmark         &\checkmark         &\checkmark         \\
Baseline Controls $\times$ $\mathbf{1}_{t\geq1920}$&\checkmark         &\checkmark         &\checkmark         &\checkmark         &\checkmark         \\
\bottomrule
\end{tabular}
}


==> output/tex/Tab_referee_2_control_pretrend.tex <==
{   \def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi} \begin{tabular}{l*{7}{c}}   \toprule  Dependent Variable & \multicolumn{7}{c}{ln(Employment)} \\    \cmidrule(lr){2-8}       
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         &\multicolumn{1}{c}{(7)}         \\
\midrule
Liab/Assets$_{i,1917}$ $\times$$\mathbf{1}_{t\geq1920}$&     62.7\sym{***}&     42.0\sym{**} &     58.8\sym{***}&     43.0\sym{**} &     54.0\sym{***}&     34.9         &     36.6\sym{*}  \\
                &   (16.0)         &   (20.5)         &   (15.6)         &   (21.3)         &   (15.9)         &   (22.0)         &   (21.1)         \\
$\Delta$ ln(Revenue)$_{i,1916-1918}$ $\times$$\mathbf{1}_{t\geq1920}$&     6.87         &     6.21         &                  &                  &                  &                  &     8.01         \\
                &   (4.68)         &   (5.39)         &                  &                  &                  &                  &   (5.52)         \\
$\Delta$ EBIT/Revenue$_{i,1916-1918}$ $\times$$\mathbf{1}_{t\geq1920}$&                  &                  &     0.13         &    -1.03         &                  &                  &    -6.14         \\
                &                  &                  &   (1.32)         &   (7.04)         &                  &                  &   (7.74)         \\
$\Delta$ FCF$_{i,1917-1918}$ $\times$$\mathbf{1}_{t\geq1920}$&                  &                  &                  &                  &    -8.26         &    -24.7\sym{*}  &    -24.0\sym{*}  \\
                &                  &                  &                  &                  &   (10.3)         &   (13.1)         &   (12.9)         \\
\midrule
Observations    &     2096         &     1796         &     2051         &     1777         &     2080         &     1813         &     1760         \\
Number of Firms &      309         &      267         &      300         &      263         &      308         &      271         &      262         \\
\(R^2_{overall}\)&     0.97         &     0.97         &     0.97         &     0.98         &     0.97         &     0.98         &     0.98         \\
\(R^2_{within}\)&    0.041         &    0.056         &    0.037         &    0.052         &    0.032         &    0.058         &    0.070         \\
Year FE         &\checkmark         &                  &\checkmark         &                  &\checkmark         &                  &                  \\
Firm FE         &\checkmark         &\checkmark         &\checkmark         &\checkmark         &\checkmark         &\checkmark         &\checkmark         \\
Controls $\times$ $\mathbf{1}_{t\geq1920}$&                  &\checkmark         &                  &\checkmark         &                  &\checkmark         &\checkmark         \\
Industry-Year-FE&                  &\checkmark         &                  &\checkmark         &                  &\checkmark         &\checkmark         \\
\bottomrule
\end{tabular}
}


==> output/tex/Tab_referee_2_past_leverage.tex <==
{   \def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}  \begin{tabular}{l*{2}{c}}   \toprule  Dependent Variable & \multicolumn{2}{c}{ln(Employment)} \\    \cmidrule(lr){2-3}       
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         \\
\midrule
Liab/Assets$_{i,1917}$ $\times$$\mathbf{1}_{t\geq1920}$&     62.4\sym{***}&     49.5\sym{**} \\
                &   (15.5)         &   (23.5)         \\
$\Delta$ Liab/Assets$_{i,1916-1917}$ $\times$$\mathbf{1}_{t\geq1920}$&    -25.8         &    -38.3         \\
                &   (30.3)         &   (37.0)         \\
\midrule
Observations    &     2308         &     1866         \\
Number of Firms &      343         &      278         \\
\(R^2_{overall}\)&     0.97         &     0.97         \\
\(R^2_{within}\)&    0.039         &    0.054         \\
Year FE         &\checkmark         &                  \\
Firm FE         &\checkmark         &\checkmark         \\
Controls $\times$ $\mathbf{1}_{t\geq1920}$&                  &\checkmark         \\
Industry-Year-FE&                  &\checkmark         \\
\bottomrule
\end{tabular}
}


==> output/tex/Tab_salings_employment_R3_exports.tex <==
{ \begin{tabular}{l*{8}{c}}   \toprule  Dependent Variable & \multicolumn{8}{c}{ln(Employment)} \\    \cmidrule(lr){2-9}       
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         &\multicolumn{1}{c}{(7)}         &\multicolumn{1}{c}{(8)}         \\
\midrule
Liab/Assets$_{i,1917} \times \mathbf{1}_{t\geq1920}$&     57.3\sym{***}&     42.0\sym{**} &     56.2\sym{***}&     37.8\sym{*}  &     66.4\sym{***}&     71.8\sym{***}&     91.4\sym{*}  &    170.7\sym{***}\\
                &   (14.3)         &   (20.9)         &   (14.1)         &   (20.4)         &   (18.3)         &   (25.0)         &   (51.6)         &   (60.2)         \\
Exporter in 1919 $\times \mathbf{1}_{t\geq1920}$&     2.58         &    -7.18         &                  &                  &                  &                  &                  &                  \\
                &   (6.55)         &   (9.72)         &                  &                  &                  &                  &                  &                  \\
Exporter in 1921 $\times \mathbf{1}_{t\geq1920}$&                  &                  &     18.3         &     41.6\sym{*}  &                  &                  &                  &                  \\
                &                  &                  &   (12.6)         &   (23.2)         &                  &                  &                  &                  \\
\midrule
Observations    &     2355         &     1866         &     2355         &     1866         &     1460         &     1194         &      288         &      220         \\
Number of Firms &      351         &      278         &      351         &      278         &      226         &      183         &       40         &       29         \\
\(R^2_{overall}\)&     0.97         &     0.97         &     0.97         &     0.98         &     0.97         &     0.97         &     0.98         &     0.98         \\
\(R^2_{within}\)&    0.033         &    0.050         &    0.038         &    0.067         &    0.050         &    0.080         &    0.092         &     0.26         \\
Year FE         &\checkmark         &                  &\checkmark         &                  &\checkmark         &\checkmark         &\checkmark         &\checkmark         \\
Firm FE         &\checkmark         &\checkmark         &\checkmark         &\checkmark         &\checkmark         &\checkmark         &\checkmark         &\checkmark         \\
Baseline Controls $\times \mathbf{1}_{t\geq1920}$&                  &\checkmark         &                  &\checkmark         &                  &\checkmark         &                  &\checkmark         \\
Industry-Year-FE&                  &\checkmark         &                  &\checkmark         &                  &                  &                  &                  \\
Sample          &All firms         &All firms         &All firms         &All firms         &Ex. mining+metal         &Ex. mining+metal         &Non-tradable         &Non-tradable         \\
\bottomrule
\end{tabular}
}


==> output/tex/Tab_war_exposure.tex <==
{ \def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}  \begin{tabular}{l*{6}{c}}   \toprule  Dependent Variable & \multicolumn{6}{c}{ln(Employment)} \\    \cmidrule(lr){2-7}       
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         \\
\midrule
Liab/Assets$_{i,1917}$ $\times$$\mathbf{1}_{t\geq1920}$&     52.6\sym{***}&     33.0\sym{*}  &     79.8\sym{***}&     57.4\sym{***}&     58.1\sym{***}&     78.7\sym{***}\\
                &   (15.2)         &   (16.9)         &   (27.5)         &   (17.3)         &   (20.1)         &   (28.2)         \\
War-relevant industry $\times \mathbf{1}_{t\geq1920} $&     7.82         &                  &                  &     6.73         &     4.01         &     1.66         \\
                &   (5.01)         &                  &                  &   (5.41)         &   (5.64)         &   (6.41)         \\
\midrule
Observations    &     2355         &     1463         &      892         &     1857         &     1660         &     1104         \\
Number of Firms &      351         &      213         &      138         &      231         &      205         &      132         \\
\(R^2_{overall}\)&     0.97         &     0.97         &     0.97         &     0.95         &     0.93         &     0.88         \\
\(R^2_{within}\)&    0.039         &   0.0097         &    0.074         &    0.041         &    0.035         &    0.051         \\
Year FE         &\checkmark         &\checkmark         &\checkmark         &\checkmark         &\checkmark         &\checkmark         \\
Firm FE         &\checkmark         &\checkmark         &\checkmark         &\checkmark         &\checkmark         &\checkmark         \\
Sample          &All firms         &w/ war-rel.         &w/o war-rel.         &<p90(size)         &<p80(size)         &<p50(size)         \\
\bottomrule
\end{tabular}
}

